Functional central limit theorems for persistent Betti numbers on cylindrical networks

We study functional central limit theorems for persistent Betti numbers obtained from networks defined on a Poisson point process. The limit is formed in large volumes of cylindrical shape stretching only in one dimension. The results cover a directed sublevel-filtration for stabilizing networks and the Cech and Vietoris-Rips complex on the random geometric graph. The presented functional central limit theorems open the door to a variety of statistical applications in topological data analysis and we consider goodness-of-fit tests in a simulation study.

==> defs.tex <==

%\normalem

\definecolor{wiasblue}   {cmyk}{1.0, 0.60, 0, 0}
\definecolor{mlugreen}{RGB}{0,81,51}


\newcommand{\blue}[1]{{\textcolor{wiasblue}{{\bf \emph{#1}}}}{}}
\newcommand{\green}[1]{{\textcolor{wiasgreen}{{\bf \emph{#1}}}}{}}
\newcommand{\mlu}[1]{{\textcolor{mlugreen}{{\bf \emph{#1}}}}{}}
\newcommand{\white}[1]{{\textcolor{white}{{\bf \emph{#1}}}}{}}
\newcommand{\red}[1]{{\textcolor{red}{{\bf \emph{#1}}}}{}}

\newcommand{\tblue}[1]{\text{\blue{$#1$}}}
\newcommand{\tgreen}[1]{\text{\green{$#1$}}}
\newcommand{\tred}[1]{\text{\red{$#1$}}}
\newcommand{\tblack}[1]{\text{{$#1$}}}

%\setbeamertemplate{bibliography item}{[\theenumiv]}

\def\Z{\mathbb Z}
\def\E{\mathbb E}
\def\P{\mathbb P}
\def\Q{\mathbb Q}
\def\R{\mathbb R}
\def\mc{\mathcal}
\def\ms{\mathsf}
\def\mf{\mathfrak}

\renewcommand\c{\mathsf{c}}
\def\CC{\mc C}


\def\rsa{\rightsquigarrow}
\def\lrsa{\leftrightsquigarrow}
\def\la{\lambda}
\def\La{\Lambda}
\def\a{\alpha}
\def\s{\sigma}
\def\su{\subset}
\def\e{\varepsilon}
\def\t{\tau}
\def\g{\gamma}
\def\b{\beta}
\def\de{\delta}
\def\ol{\overline}
\def\om{\omega}
\def\Om{\Omega}
\def\es{\emptyset}
\def\one{\mathbbmss{1}}
\def\tw{\textcolor{white}{.}}
\def\Gl{G^{\ms L}}
\def\Gr{G^{\ms R}}
\def\Gd{G^\De}
\def\De{\Delta}
\def\const{\ms{const}}
\def\ff{\infty}
\def\Ra{\Rightarrow}
\def\lc{\lceil}
\def\rc{\rceil}
\def\mt{\mapsto}
\def\vp{\varphi}
\def\cd{\cdots}
\def\Poi{\ms{Poi}}
\def\Exp{\ms{Exp}}
\def\Leb{\ms{Leb}}
\def\d{{\rm d}}
\def\k{\kappa}
\def\EE{\mc E}
\def\LL{\mc L}
\def\HH{\mc H}
\def\PP{\mc P}
\def\FF{\mc F}
\def\FFo{\mc F^o}
\def\lc{\lceil}
\def\rc{\rceil}
\def\lf{\lfloor}
\def\rf{\rfloor}
\def\ls{\limsup}
\def\f{\frac}
\def\lan{\langle}
\def\ran{\rangle}
\def\xra{\xrightarrow}
\def\NN{\mc N}
\def\cd{\cdots}
\def\off{[0,\ff)}
\def\r{\rho}
\def\ua{\uparrow}
\def\be{\begin}
\def\en{\end}
\def\im{\item}
\def\sm{\setminus}
\def\th{\theta}
\def\bep{\begin{proof}}
\def\enp{\end{proof}}
\def\bepr{\begin{proposition}}
\def\enpr{\end{proposition}}
\def\bec{\begin{corollary}}
\def\enc{\end{corollary}}
\def\bea{\begin{align}}
\newcommand\eea{\end{align}}
\def\beas{\begin{align*}}
\def\eeas{\end{align*}}
\def\bet{\begin{theorem}}
\def\ent{\end{theorem}}
\def\bee{\begin{example}}
\def\ene{\end{example}}
\def\zz{\ms z}
\def\da{\downarrow}
\def\bede{\begin{definition}}
\def\ende{\end{definition}}
\def\been{\begin{enumerate}}
\def\enen{\end{enumerate}}
\def\li{\liminf}
\def\ls{\limsup}
\def\w{\wedge}
\def\i{{\ms i}}

